Direct Comparison of Magnetic Penetration Depth in Kagome Superconductors AV$_3$Sb$_5$ (A = Cs, K, Rb)

We report measurements of the local temperature-dependent penetration depth, $\lambda(T)$, in the Kagome superconductors AV$_3$Sb$_5$ (A = Cs, K, Rb) using scanning superconducting quantum interference device (SQUID) microscopy. Our results suggest that the superconducting order in all three compounds is fully gapped, in contrast to reports of nodal superconductivity in KV$_3$Sb$_5$ and RbV$_3$Sb$_5$. Analysis of the temperature-dependent superfluid density, $\rho_s(T)$, shows deviations from the behavior expected for a single isotropic gap, but the data are well described by models incorporating either a single anisotropic gap or two isotropic gaps. Notably, the temperature dependences of $\lambda(T)$ and $\rho_s(T)$ in KV$_3$Sb$_5$ and RbV$_3$Sb$_5$ are qualitatively more similar to each other than to CsV$_3$Sb$_5$, consistent with the superconducting phase reflecting features of the normal-state band structure. Our findings provide a direct comparison of the superconducting properties across the AV$_3$Sb$_5$ family.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx2.tex <==


